MINOS: Multimodal Indoor Simulator for Navigation in Complex Environments

We present MINOS, a simulator designed to support the development of multisensory models for goal-directed navigation in complex indoor environments. The simulator leverages large datasets of complex 3D environments and supports flexible configuration of multimodal sensor suites. We use MINOS to benchmark deep-learning-based navigation methods, to analyze the influence of environmental complexity on navigation performance, and to carry out a controlled study of multimodality in sensorimotor learning. The experiments show that current deep reinforcement learning approaches fail in large realistic environments. The experiments also indicate that multimodality is beneficial in learning to navigate cluttered scenes. MINOS is released open-source to the research community at http://minosworld.org . A video that shows MINOS can be found at https://youtu.be/c0mL9K64q84

==> figures_tex/fig_action_traces.tex <==
%!TEX root = main.tex

\begin{figure*}
\includegraphics[width=.24\textwidth]{images/traces/114cf5e77612f4b282007f1bca6c07a1_84.png}\hfill
\includegraphics[width=.24\textwidth]{images/traces/676d627de72e97978a0e72c9b3894621_48.png}\hfill
\includegraphics[width=.24\textwidth]{images/traces/5da2a081094d905866c46fc6c87326ce_61.png}\hfill
\includegraphics[width=.24\textwidth]{images/traces/c72a1b427ea3d5a615ecc65e0ae034f1_65.png}\\
\includegraphics[width=.24\textwidth]{images/traces/722e25bc5f193527902e65aa9b432268_72.png}\hfill
\includegraphics[width=.24\textwidth]{images/traces/9dccca3f5696dcab416f952bdb807755_78.png}\hfill
\includegraphics[width=.24\textwidth]{images/traces/e3310eacee95df7b6b5ddd748840a424_9.png}\hfill
\includegraphics[width=.24\textwidth]{images/traces/3eb0be5f8a986b39fb6b7e00d31ee2b9_58.png}
\caption{Example navigation episodes for the full multimodal agent in furnished environments, visualized from an overhead view (nonphotorealistic rendering, walls in blue).  The goal door is highlighted in green, and the agent's trajectory is shown in orange.  Red lines on the trajectory indicate the direction of sensed contact forces. (Zoom in to see these.) The shortest path between the start and goal positions is visualized with blue tiles.  The episode in the bottom right is a failure case where the agent is trapped behind a U-shaped kitchen island.}
\label{fig:action_traces}
\vspace{-3mm}
\end{figure*}


==> figures_tex/fig_dfp_complexity_train_curves.tex <==
%!TEX root = ../main.tex

\begin{figure}
\includegraphics[width=\textwidth]{images/dfp_complexity_train_curves.pdf}
\caption{\alexey{Do we need this figure? If yes, do we need the "speed"?} Performance of DFP-based agent on environments of different size and complexity. MP3D-S and MP3D-M are Matterport3D houses with up to 10 rooms and up to 24 rooms respectively.  SUNCG-SF and SUNCG-MF are small and medium-sized SUNCG houses with two rooms and three to five rooms respectively.  SUNCG-SE and SUNCG-ME are the same houses with all furniture removed, creating empty maze-like environments.  The average episode success and speed for four runs are plotted.  Note that final trained performance degrades drastically with increasing environment size and environment clutter level.}
\label{fig:dfp_complexity_train_curves}
\end{figure}


==> figures_tex/fig_dist_plot.tex <==
%!TEX root = main.tex
\begin{figure}
\includegraphics[width=\linewidth]{images/dist_plot.pdf}
\caption{Performance of trained agents as a function of distance between the start and goal positions.  Agent performance degrades as distance to the goal increases.}
%  The multimodal agents (M+V+F and M+V+D+F) combine the short-range performance advantage of the touch modality with the long-range performance advantages of depth and visual perception.}
\label{fig:dist_plot}
\vspace{-3mm}
\end{figure}


==> figures_tex/fig_sim_architecture.tex <==
%!TEX root = main.tex
\begin{figure*}
\caption{\todo{Create block architecture diagram}}
\label{fig:sim_architecture}
\end{figure*}


==> figures_tex/fig_train_curves.tex <==
%!TEX root = supplemental.tex

\begin{figure}[hb]
\includegraphics[width=\textwidth]{images/train_curves.pdf}
\caption{Performance of indoor navigation agents with different multimodal input combinations. Training episodes are randomly sampled from the furnished house training set.}
\label{fig:train_curves}
\end{figure}


==> figures_tex/tab_audio_results.tex <==
%!TEX root = main.tex
\begin{table*}[ht]
	\centering
	\begin{tabular}{@{}llcccc@{}}
	\toprule
	 & & \multicolumn{2}{c}{empty room} & \multicolumn{2}{c}{furnished room} \\
	\cmidrule(lr){3-4} \cmidrule(lr){5-6}
	input modality & prediction target & success & speed & success & speed \\
	\midrule
	measurements & measurements & 90.6 & 68.1 & 46.2 & 27.2 \\
	audio & measurements & 83.1 & 61.0 & 33.8 & 22.2 \\
	audio & audio & 82.3 & 60.5 & 29.6 & 18.4 \\
	\bottomrule
	\end{tabular}
\vspace{1mm}
	\caption{Task performance in empty and furnished rooms when audio input is used in place of GPS-like measurements of the agent's position relative to the goal.}
	\label{tab:audio_results}
\vspace{-3mm}
\end{table*}


==> figures_tex/tab_force_ablation.tex <==
%!TEX root = main.tex
\begin{table*}
	\centering
	\begin{tabular}{@{}lcccc@{}}
	\toprule
	 & no prediction target & raw force & total force & force mean windows \\
	\midrule
	Success & 49.8 & 51.6 & 20.0 & \textbf{56.0} \\
	\bottomrule
	\end{tabular}
\vspace{1mm}
	\caption{Average success rate in furnished rooms for different contact force prediction targets.}
	\label{tab:force_ablation}
\vspace{-5mm}
\end{table*}


==> figures_tex/tab_history_ablation.tex <==
%!TEX root = supplemental.tex

\begin{table}[hb]
	\centering
	\begin{tabular}{@{}lccccc@{}}
	\toprule
	 & no history & 2 frames  & 4 frames & 8 frames & 16 frames \\
	\midrule
	Episode success rate & 37.8 & 41.1 & \textbf{56.0} & 47.1 & 42.1 \\
	\bottomrule
	\end{tabular}
	\vspace{1mm}
	\caption{Average success rate for force and measurements agent in the furnished house scenario using different input history lengths.}
	\label{tab:history_ablation}
	\vspace{-3mm}
\end{table}


==> tex/acknowledgments.tex <==
%!TEX root = main.tex
\todo{Acknowledgments go here.}

